GLASSES: Relieving The Myopia Of Bayesian Optimisation

We present GLASSES: Global optimisation with Look-Ahead through Stochastic Simulation and Expected-loss Search. The majority of global optimisation approaches in use are myopic, in only considering the impact of the next function value; the non-myopic approaches that do exist are able to consider only a handful of future evaluations. Our novel algorithm, GLASSES, permits the consideration of dozens of evaluations into the future. This is done by approximating the ideal look-ahead loss function, which is expensive to evaluate, by a cheaper alternative in which the future steps of the algorithm are simulated beforehand. An Expectation Propagation algorithm is used to compute the expected value of the loss.We show that the far-horizon planning thus enabled leads to substantive performance gains in empirical tests.

==> definitions.tex <==
% This file defines macros, notation is defined in notationDef.tex
\usepackage{color}
\usepackage{verbatim}

\global\long\def\neil#1{\textbf{\color{red}#1}}
%\global\long\def\todo#1{\textbf{TODO: #1}}
\global\long\def\instructions#1{\textbf{INSTRUCTIONS: #1}}

\definecolor{brown}{rgb}{0.9,0.59,0.078}
\definecolor{ironsulf}{rgb}{0,0.7,.5}
\definecolor{lightpurple}{rgb}{0.156,0,0.245}

\newenvironment{matlab}{\comment}{\endcomment}
\newenvironment{octave}{\comment}{\endcomment}
\newenvironment{matlabv}{\verbatim}{\endverbatim}
\newenvironment{octavev}{\verbatim}{\endverbatim}

\ifdefined\blackBackground
\definecolor{colorOne}{rgb}{0, 1, 1}
\definecolor{colorTwo}{rgb}{1, 0, 1}
\definecolor{colorThree}{rgb}{1, 1, 0}
\definecolor{colorTwoThree}{rgb}{1, 0, 0}
\definecolor{colorOneThree}{rgb}{0, 1, 0}
\definecolor{colorOneTwo}{rgb}{0, 0, 1}
\else
\definecolor{colorOne}{rgb}{1, 0, 0}
\definecolor{colorTwo}{rgb}{0, 1, 0}
\definecolor{colorThree}{rgb}{0, 0, 1}
\definecolor{colorTwoThree}{rgb}{0, 1, 1}
\definecolor{colorOneThree}{rgb}{1, 0, 1}
\definecolor{colorOneTwo}{rgb}{1, 1, 0}
\fi

\ifdefined\blackBackground
\global\long\def\redColor{cyan}
\global\long\def\greenColor{magenta}
\global\long\def\blueColor{yellow}
\global\long\def\magentaColor{green}
\global\long\def\blackColor{white}
\global\long\def\whiteColor{black}
\else
\global\long\def\redColor{red}
\global\long\def\greenColor{green}
\global\long\def\blueColor{blue}
\global\long\def\magentaColor{magenta}
\global\long\def\blackColor{black}
\global\long\def\whiteColor{white}
\fi

\global\long\def\det#1{\left|#1\right|}
\global\long\def\erf{\text{erf}}
\global\long\def\refeq#1{(\ref{#1})}
\global\long\def\refsec#1{Section \ref{#1}}
\global\long\def\refsecs#1#2{Sections \ref{#1}--\ref{#2}}
\global\long\def\reftwosec#1#2{Sections \ref{#1} and \ref{#2}}
\global\long\def\Refsec#1{Section \ref{#1}}

% Try and avoid these macros for notation, they are definitions of convenience.
\global\long\def\bfdelta{\boldsymbol{\delta}}
\global\long\def\bfDelta{\boldsymbol{\Delta}}
\global\long\def\bfbeta{\boldsymbol{\beta}}
\global\long\def\bfgamma{\boldsymbol{\gamma}}
\global\long\def\bfmu{\boldsymbol{\mu}}
\global\long\def\bfnu{\boldsymbol{\nu}}
\global\long\def\bfalpha{\boldsymbol{\alpha}}
\global\long\def\bfepsilon{\boldsymbol{\epsilon}}
\global\long\def\bfSigma{\boldsymbol{\Sigma}}
\global\long\def\bftau{\boldsymbol{\tau}}
\global\long\def\bflambda{\boldsymbol{\lambda}}
\global\long\def\bfLambda{\boldsymbol{\Lambda}}
\global\long\def\bfpsi{\boldsymbol{\psi}}
\global\long\def\bfxi{\boldsymbol{\xi}}
\global\long\def\bfpi{\bm{\pi}}
\global\long\def\bfPsi{\boldsymbol{\Psi}}
\global\long\def\bfphi{\boldsymbol{\phi}}
\global\long\def\bfPhi{\boldsymbol{\Phi}}
\global\long\def\bfrho{\boldsymbol{\rho}}
\global\long\def\bftheta{\boldsymbol{\theta}}
\global\long\def\bfTheta{\boldsymbol{\Theta}}
\global\long\def\bfomega{\boldsymbol{\omega}}


\global\long\def\Bmath#1{\boldsymbol{#1}}


% Avoid these macros for notation, they are definitions of convenience.
\global\long\def\bfa{\mathbf{a}}
\global\long\def\bfb{\mathbf{b}}
\global\long\def\bfc{\mathbf{c}}
\global\long\def\bfd{\mathbf{d}}
\global\long\def\bfe{\mathbf{e}}
\global\long\def\bff{\mathbf{f}}
\global\long\def\bfg{\mathbf{g}}
\global\long\def\bfh{\mathbf{h}}
\global\long\def\bfk{\mathbf{k}}
\global\long\def\bfl{\mathbf{l}}
\global\long\def\bfm{\mathbf{m}}
\global\long\def\bfn{\mathbf{n}}
\global\long\def\bfo{\mathbf{o}}
\global\long\def\bfp{\mathbf{p}}
\global\long\def\bfq{\mathbf{q}}
\global\long\def\bfr{\mathbf{r}}
\global\long\def\bfs{\mathbf{s}}
\global\long\def\bft{\mathbf{t}}
\global\long\def\bfu{\mathbf{u}}
\global\long\def\bfv{\mathbf{v}}
\global\long\def\bfw{\mathbf{w}}
\global\long\def\bfx{\mathbf{x}}
\global\long\def\bfy{\mathbf{y}}
\global\long\def\bfz{\mathbf{z}}

\newcommand{\dif}[1]{\text{d}#1}
\global\long\def\cov{\text{cov}}


\global\long\def\bfzero{\mathbf{0}}
\global\long\def\bfone{\mathbf{1}}


\global\long\def\bfA{\mathbf{A}}
\global\long\def\bfB{\mathbf{B}}
\global\long\def\bfC{\mathbf{C}}
\global\long\def\bfD{\mathbf{D}}
\global\long\def\bfE{\mathbf{E}}
\global\long\def\bfG{\mathbf{G}}
\global\long\def\bfH{\mathbf{H}}
\global\long\def\bfI{\mathbf{I}}
\global\long\def\eye{\mathbf{I}}
\global\long\def\bfK{\mathbf{K}}
\global\long\def\bfL{\mathbf{L}}
\global\long\def\bfM{\mathbf{M}}
\global\long\def\bfO{\mathbf{O}}
\global\long\def\bfP{\mathbf{P}}
\global\long\def\bfQ{\mathbf{Q}}
\global\long\def\bfR{\mathbf{R}}
\global\long\def\bfS{\mathbf{S}}
\global\long\def\bfT{\mathbf{T}}
\global\long\def\bfU{\mathbf{U}}
\global\long\def\bfV{\mathbf{V}}
\global\long\def\bfW{\mathbf{W}}
\global\long\def\bfX{\mathbf{X}}
\global\long\def\bfY{\mathbf{Y}}
\global\long\def\bfZ{\mathbf{Z}}
\global\long\def\llangle{{\langle\vspace{-2mm} \langle}}
\global\long\def\rrangle{{\rangle\vspace{-2mm} \rangle}}
\global\long\def\la{\leftarrow}


\global\long\def\tf{\tilde{f}}
\global\long\def\tg{\tilde{g}}
\global\long\def\tX{\tilde{X}}
\global\long\def\tY{\tilde{Y}}
\global\long\def\tZ{\tilde{Z}}


\global\long\def\bbE{\mathbb{E}}
\global\long\def\bbR{\mathbb{R}}
\global\long\def\bbP{\mathbb{P}}
\global\long\def\bbT{\mathbb{T}}
\global\long\def\bbZ{\mathbb{Z}}


\global\long\def\ois{2 \pi i s}
\global\long\def\oik{2 \pi i k}
\global\long\def\oin{2 \pi i n}
\global\long\def\oim{2 \pi i m}


\global\long\def\T{{\top}}
\global\long\def\Tr{\mbox{Tr}}
\global\long\def\trace#1{\text{tr}\left(#1\right)}
%\global\long\def\diff#1{{\, d#1}}
\global\long\def\diff#1#2{\frac{\text{d}#1}{\text{d}#2}}
\global\long\def\vgraph#1{ \newpage\begin{center} \end{center}{center}{center}{center}{center}{center}{center}{center}{center}{center}{center}{center}{center}{center}{center}{center}{center} {\large{\bf #1}} {center} \vspace{2mm} }
\global\long\def\high#1{\textcolor{blue}{\emph{#1}}}
\global\long\def\cut#1{}
\global\long\def\citeasnoun#1{\citeN{#1}}
\global\long\def\citemulti#1#2{(#1, \citeyearNP{#2})}
\global\long\def\citemultiN#1#2{#1 (\citeyearNP{#2})}
\global\long\def\Sum{{\displaystyle \sum}}
\global\long\def\defeq{{\stackrel{def}{=}}}
\global\long\def\marg#1{\marginpar{#1}}


\global\long\def\pdt#1#2{\frac{\partial^{2} #1}{\partial{#2}^{2} }}
\global\long\def\pdsd#1#2#3{\frac{\partial^{2} #1}{\partial{#2} \partial{#3} }}
\global\long\def\pdo#1#2{\frac{\partial{#1}}{\partial{#2}}}
\global\long\def\pdol#1#2{\partial{#1}/ \partial{#2}}
\global\long\def\pdu#1{\frac{\partial}{\partial{#1}}}

\global\long\def\reffig#1{figure~\ref{#1}}
\global\long\def\Reffig#1{Figure~\ref{#1}}
\global\long\def\reffigrange#1#2{figure~\ref{#1}--\ref{#2}}
\global\long\def\Reffigrange#1#2{Figure~\ref{#1}--\ref{#2}}
\global\long\def\refbox#1{box~\ref{#1}}
\global\long\def\Refbox#1{Box~\ref{#1}}
\global\long\def\refeqs#1#2{equation~(\ref{#1})--(\ref{#2})}
\global\long\def\Refeqs#1#2{Equation~(\ref{#1})--(\ref{#2})}
\global\long\def\reftip#1{tip~\ref{#1}}
\global\long\def\Reftip#1{Tip~\ref{#1}}
\global\long\def\refint#1{intuition~\ref{#1}}
\global\long\def\Refint#1{Intuition~\ref{#1}}
\global\long\def\reftable#1{table~\ref{#1}}
\global\long\def\Reftable#1{Table~\ref{#1}}
\global\long\def\refchap#1{chapter~\ref{#1}}
\global\long\def\Refchap#1{Chapter~\ref{#1}}
\global\long\def\refapp#1{appendix~\ref{#1}}
\global\long\def\Refappendix#1{Appendix~\ref{#1}}
\global\long\def\refchaprange#1#2{chapter~\ref{#1}--\ref{#2}}
\global\long\def\Refchaprange#1#2{Chapter~\ref{#1}--\ref{#2}}
\global\long\def\refsection#1{section~\ref{#1}}
\global\long\def\Refsection#1{Section~\ref{#1}}

\global\long\def\fixme#1{\emph{\textbf{#1}}}

\global\long\def\detail#1{}

% For putting a footer when an include is made.
\global\long\def\includetalkfile#1{{\setbeamertemplate{footline}{\url{#1} \hfill \insertframenumber} \input{#1}}}

%\global\long\def\includetalkfile#1{\input{#1}}
\global\long\def\newsection#1#2{\section{#1}\begin{frame}\frametitle{Outline}\tableofcontents[currentsection,hideallsubsections]\end{frame}\includetalkfile{#2}}

\global\long\def\inputdiagram#1{{\small\input{#1}\vspace{0.5cm}}}

\global\long\def\newsubsection#1#2{\subsection{#1}\includetalkfile{#2}}
\global\long\def\newsubsubsection#1#2{\subsubsection{#1}\includetalkfile{#2}}


\global\long\def\includecvfile#1{\input{#1}}
\global\long\def\newcvsection#1#2{\section*{#1}\includecvfile{#2}}

\global\long\def\newcvsubsection#1#2{\subsection*{#1}\includecvfile{#2}}
\global\long\def\newcvsubsubsection#1#2{\subsubsection*{#1}\includecvfile{#2}}
\global\long\def\newcvparagraph#1#2{\paragraph{#1}\includecvfile{#2}}

\global\long\def\twoimageslidewidth#1#2#3#4{\begin{frame}[plain]
  \begin{center}
    \href{#3}{\includegraphics[width=0.45\textwidth]{#1}}\hfill
    \href{#3}{\includegraphics[width=0.45\textwidth]{#2}}
  \end{center}
\end{frame}
\note{#4}}
\global\long\def\imageslidewidth#1#2#3{\begin{frame}[plain]
  \begin{center}
    \href{#2}{\includegraphics[width=0.9\textwidth]{#1}}
  \end{center}
\end{frame}
\note{#3}}
\global\long\def\imageslideheight#1#2#3{\begin{frame}[plain]
  \begin{center}
    \href{#2}{\includegraphics[height=0.9\textheight]{#1}}
  \end{center}
\end{frame}
\note{#3}}

\global\long\def\paperslide#1#2#3{\begin{frame}[plain]
  \begin{center}
    {\setlength\fboxsep{0pt}%
      \colorbox{white}{
    \href{#2}{\includegraphics[trim=0cm 20cm 0cm 0cm, clip=true, width=\textwidth]{#1}}}
    }
  \end{center}
\end{frame}
\note{#3}}




==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


